Subfactors, Planar Algebras and Rotations

Growing out of the initial connections between subfactors and knot theory that gave rise to the Jones polynomial, Jones' axiomatization of the standard invariant of an extremal finite index $II_1$ subfactor as a spherical $C^*$-planar algebra, presented in arXiv:math.QA/9909027, is the most elegant and powerful description available. We make the natural extension of this axiomatization to the case of finite index subfactors of arbitrary type. We also provide the first steps toward a limited planar structure in the infinite index case. The central role of rotations, which provide the main non-trivial part of the planar structure, is a recurring theme throughout this work. In the finite index case the axioms of a $C^*$-planar algebra need to be weakened to disallow rotation of internal discs, giving rise to the notion of a rigid $C^*$-planar algebra. We show that the standard invariant of any finite index subfactor has a rigid $C^*$-planar algebra structure. We then show that rotations can be re-introduced with associated correction terms entirely controlled by the Radon-Nikodym derivative of the two canonical states on the first relative commutant, $N' \cap M$. By deforming a rigid $C^*$-planar algebra to obtain a spherical $C^*$-planar algebra and lifting the inverse construction to the subfactor level we show that any rigid $C^*$-planar algebra arises as the standard invariant of a finite index $II_1$ subfactor equipped with a conditional expectation, which in general is not trace preserving. Jones' results thus extend completely to the general finite index case. We conclude by applying our machinery to the $II_1$ case, shedding new light on the rotations studied by Huang [11] and touching briefly on the work of Popa [29]. (continued in article)

==> inf/Ncentral.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% N-Central Vectors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{$N$-Central Vectors}
\label{sect: N-central vectors}

Here we will show that the set of $N$-central vectors in $\Ltwo(M_k)$
is $\overline{N' \cap \gothn_{\Trace_k}}$ (closure in $\Ltwo(M_k)$).
The proof is essentially an application of ideas from
Popa~\cite{Popa1981}.

\begin{definition}
$\xi\in\Ltwo(M_k)$ is an {\em $N$-central vector} if $n\xi=\xi n$ for
all $n\in N$.  The set of $N$-central vectors in $\Ltwo(M_k)$ is
denoted $N' \cap \Ltwo(M_k)$.
\end{definition}

\begin{lemma}
\label{2-norm lsc}
Let $M$ be a semifinite von Neumann algebras with n.f.s trace $\Trace$.
The 2-norm $||x||_2=[\Trace(x^*x)]^{1/2}$ is lower
semi-continuous with respect to the weak operator topology.
\begin{proof}
Suppose $\{ y_{\alpha} \}$ is a net in $M$ converging weakly to $y$.
Take a set of orthogonal projections $\{ p_k \} \subset
\gothn_{\Trace}$ with $\sum p_k =1$.  Then for $z\in \gothn_{\Trace}$
with $|| z ||_2\leq 1$ one has $|< y_{\alpha}
\hatt{p_k},\hatt{z}>|\leq || y_{\alpha} p_k||_2$ and hence
\[
|<y\hatt{p_k},\hatt{z}>|=\lim |< y_{\alpha} \hatt{p_k},\hatt{z}>|
	\leq \liminf_{\alpha} ||y_{\alpha} p_k ||_2
\]
so that
\[
||y p_k||_2
 =\sup\{|<y\hatt{p_k},\hatt{z}>| : z\in {\gothn_{\Trace}}, ||z||_2\leq 1 \}
 \leq \liminf ||y_{\alpha} p_k||_2 .	
\]
Finally, using Fatou's lemma for the second inequality,
\[
||y||_2^2=\sum_k ||y p_k||_2^2
	\leq \sum_k \liminf_{\alpha} ||y_{\alpha} p_k||_2^2
	\leq \liminf_{\alpha} \sum_k ||y_{\alpha} p_k||_2^2
	= \liminf_{\alpha} ||y_{\alpha}||_2^2 .
\]
\end{proof}
\end{lemma}

\begin{remark}
The fact that $||y||_2^2=\sum_k ||y p_k||_2^2$ even if $y\notin
\gothn_{\Trace}$ is established as follows.  Let
$q_N=\sum_{k=1}^N{p_k}$ and note that $q_N\nearrow 1$.  Hence
$yq_Ny^*\nearrow yy^*$ and so $Tr(q_Ny^*yq_N)= Tr(yq_N y^*)\nearrow
Tr(yy^*)=||y||_2^2$ (even though $q_Ny^*yq_N$ may {\em not} be
increasing).  Finally, $y^*yq_N\in \gothn_{\Trace}$ and
$Tr(q_Ny^*yq_N)=Tr(y^*yq_N)=\sum_{k=1}^N Tr(y^*yp_k)=\sum_{k=1}^N
||yp_k||_2^2$.
\end{remark}


The next lemma follows exactly the line of proof in
Popa~\cite{Popa1981} 2.3.

\begin{prop}
\label{convex averaging}
Let $N$ be a von Neumann subalgebra of a semifinite von Neumann
algebra $M$ equipped with a n.f.s. trace $\Trace$.  Let ${\mathcal
U}(N)$ denote the unitary group of $N$.  Let $x\in \gothn_{\Trace}$
and let $K_0=\{ \sum_{i=1}^n \lambda_i v_i x v_i^* : \lambda_i
\in[0,\infty], \sum \lambda_i=1, v_i\in {\mathcal U}(N) \}$.  Then
$N'\cap {\gothn_{\Trace}}\cap \overline{K_0}\neq \emptyset$, where
$\overline{K_0}$ denotes the weak closure of $K_0$.
\begin{proof}
Let $K=\overline{K_0}$.  Observe that for $v_i\in {\mathcal U}(N)$ and
$\lambda_i\in[0,\infty]$ such that $\sum\lambda_i=1$, we have
$||\sum_{i=1}^n \lambda_i v_i x v_i^* || \leq \sum_{i=1}^n \lambda_i
||v_ix v_i^* || = \sum_{i=1}^n \lambda_i ||x|| = ||x||$.  Hence
$K\subset B(0, ||x||)$ ($||y||=\sup\{ |<y\xi,\eta >|: \xi, \eta \in
({\mathcal H})_1\}$, so if $y_{\alpha}\rightarrow y$ and
$||y_{\alpha}||\leq r$ for all $\alpha$ then $||y||\leq r$).

Since $K$ is bounded and weakly closed it is weakly compact.  Let
$\omega=\inf_K {||y||_2}$ (note that $\omega<\infty$ since $x\in K$).
Take $y_n\in K$ such that $||y_n||_2\rightarrow \omega$.  Since $K$ is
weakly compact there exists a weakly convergent subsequence.  Hence we
may assume that $\{ y_n \}$ is weakly convergent.  Let $y=\lim y_n$.

Since $||\cdot ||_2$ is lower semi-continuous for the weak operator
topology we have $\omega\leq ||y||_2 \leq \liminf ||y_n||_2 = \omega$
and hence $||y||_2=\omega$.

Since $K$ is convex $y$ is the unique element of $K$ such that
$||y||_2=\omega$, for if $||y||_2=||z||_2=\omega$ then
$\frac{1}{2}(y+z)\in K$ so
\[
\omega^2\leq \frac{1}{4} ||y+z||^2=\frac{1}{2}\omega^2+\frac{1}{2}{\mathrm Re}
<y,z>
	\leq \frac{1}{2}\omega^2+\frac{1}{2}||y||_2||z||_2
	=\omega^2
\]
with equality iff $y=z$.

Finally, note that for all $v\in {\mathcal U}(N)$ we have $vyv^*\in K$
and $||vyv^*||_2=||y||_2$ so that $vyv^*=y$.  Hence $y\in N'\cap M$,
and since $||y||_2=\omega<\infty$, $y\in \gothn_{\Trace}$.
\end{proof}
\end{prop}


\begin{cor}
\label{cor: almost N'}
Let $N$ be a von Neumann subalgebra of a semifinite von Neumann
algebra $M$ equipped with a n.f.s. trace $\Trace$ and suppose that
$x\in M$ and $||uxu^*-x||_2\leq\delta$ for all $u\in {\mathcal U}(N)$.
Then there exists $y\in N'\cap M$ with $||x-y||_2\leq \delta$.
\begin{proof}
Let $v_i\in {\mathcal U}(N)$ and let $\lambda_i \in[0,1]$ such that
$\sum\lambda_i=1$.  Then
\[
||\sum \lambda_i v_i x v_i^*-x||_2
	=||\sum \lambda_i (v_i x v_i^*-x)||_2
	\leq \sum \lambda_i ||v_i x v_i^*-x||_2
	\leq \sum \lambda_i \delta
	= \delta
\]
So $||x-z||_2\leq\delta$ for all $z\in K_0$.  By the previous lemma
there exists $y\in N'\cap M$ and $\{y_n\}$ in $K_0$ with
$y_n\rightarrow y$ weakly.  Thus $x-y_n\rightarrow x-y$ weakly and by
the lower semi-continuity of $||\cdot ||_2$
\[
||x-y||_2\leq \liminf ||x-y_n||_2 \leq \delta .
\]
\end{proof}
\end{cor}


\begin{thm}
\label{L2=rel comm + commutators}
Let $N$ be a von Neumann subalgebra of a semifinite von Neumann
algebra $M$ equipped with a n.f.s. trace $\Trace$.  Then
\begin{description}
\item{(i)} $N' \cap \Ltwo(M)=\overline{N' \cap \gothn_{\Trace}}$.
\item{(ii)} $\br{N' \cap \Ltwo(M)}^\perp$ is the (span of) the
commutators in $\Ltwo(M)$.  Hence
\[
{\mathrm L}^2(M)=\overline{N'\cap {\gothn_{\Trace}}}\oplus
\overline{[\gothn_{\Trace},N]} .
\]
\end{description}
\begin{proof}
\begin{description}
\item{(i)} Clearly $N'\cap \gothn_{\Trace} \subseteq N'\cap\Ltwo(M)$.
Let $\xi\in N'\cap\Ltwo(M)$.  Take $\{ x_m \}$ in $\gothn_{\Trace}$
with $\hatt{x_m}\rightarrow \xi$ in $||\cdot||_2$.  Then for all $u\in
{\mathcal U}(N)$
\begin{multline*}
||ux_mu^*-x_m||_2
=||ux_m-x_mu||_2
=||u(x_m-\xi)-(x_m-\xi)u||_2 \\
 \leq ||u(x_m-\xi)||_2 +||(x_m-\xi)u||_2
 =2||x_m-\xi||_2
\end{multline*}

By Corollary~\ref{cor: almost N'} there are $y_m\in N'\cap
\gothn_{\Trace}$ with $||x_m-y_m||\leq 2||x_m-\xi||_2$ and thus
$||y_m-\xi||_2\leq 4 ||x_m-\xi||_2 \rightarrow 0$.  Thus $\xi\in
\overline{N'\cap \mathcal N}$, so ${N'\cap\Ltwo(M)}=\overline{N'\cap
\gothn_{\Trace}}$.
\item{(ii)} Simply note that 
$<\xi,n\hatt{m}-\hatt{m}n>=<n^* \xi-\xi n^*,\hatt{m}>$, so $\xi \in
N'\cap\Ltwo(M)$ iff $\xi \perp [\mathfrak{N},N]$.
\end{description}
\end{proof}
\end{thm}


\begin{cor}
\label{L2=rel comm + commutators, finite index}
If $N\subset M$ is a finite index $\IIone$ subfactor then the
$N$-central vectors in $\Ltwo(M_k)$ are precisely $N' \cap M_k$.
\begin{proof}
$\gothn_{\Trace}=M_k$ and $N' \cap M_k$ is finite dimensional so
$\overline{N' \cap M_k}=N' \cap M_k$.
\end{proof}
\end{cor}

\begin{cor}
\label{pcentral via strong limits of convex average}
Let $x\in \gothn_{\Trace}$ and let $K_0=\{ \sum_{i=1}^n \lambda_i v_i
x v_i^* : \lambda_i \in[0,\infty], \sum \lambda_i=1, v_i\in {\mathcal
U}(N) \}$.  Then $P_{N'\cap\Ltwo(M)}(x)$ is in the strong closure of
$K_0$.
\begin{proof}
We will show that the element $y \in N' \cap \gothn_{\Trace} \cap
\overline{K_0}$ whose existence is guaranteed by Prop~\ref{convex
averaging} is $P_{N'\cap\Ltwo(M)}(x)$.  Since $K_0$ is convex its weak
and strong closures coincide.

Note that for all $z \in N' \cap \gothn_{\Trace}$,
\[
\sum_{i=1}^n \ip{\lambda_i v_i x v_i^*, z}
=\sum_{i=1}^n \lambda_i \ip{x, v_i^* z v_i}
=\sum_{i=1}^n \lambda_i \ip{x,z}
=\ip{x,z} .
\]
Take $y_{\alpha}$ in $K_0$ such that $y_{\alpha} \rightarrow y$
weakly.  Then for all $z_1, z_2 \in N' \cap \gothn_{\Trace}$
\[
\ip{y, z_1 z_2^*}
=\ip{y \hatt{z_2},\hatt{z_1}}
=\lim_{\alpha} \ip{y_{\alpha} \hatt{z_2},\hatt{z_1}}
=\lim_{\alpha} \ip{y_{\alpha}, z_1 z_2^*}
=\ip{x,z_1 z_2^*} .
\]
Since $\{ z_1 z_2^* : z_i \in N' \cap \gothn_{\Trace}\}$ is dense in
$N'\cap\Ltwo(M)$, $y=P_{N'\cap\Ltwo(M)}(x)$.

The density of $\{ z_1 z_2^* : z_i \in N' \cap \gothn_{\Trace}\}$ in
$\overline{N' \cap \gothn_{\Trace}}$ can be seen as follows.  By
Takesaki~\cite{Takesaki1979}, Chapter V, Lemma 2.13, there exists a
maximal central projection $p$ of $N' \cap M$ such that $\Trace$ is
semifinite on $p(N' \cap M)$ and $\Trace=\infty$ on $[(1-p)(N' \cap
M)]_+\backslash \{ 0 \}$.  Let $A=p(N' \cap M)$.  Then
$\gothn_{\Trace_A}=N' \cap \gothn_{\Trace}$ and $\Ltwo(A)=\overline{N'
\cap \gothn_{\Trace}}$.  By Tomita-Takesaki theory applied to
$(A,\Trace)$ we see that $\{ z_1 z_2^* : z_i \in \gothn_{\Trace_A}\}$
is dense in $\Ltwo(A)$.
\end{proof}
\end{cor}


==> inf/extremality.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% EXTREMALITY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Extremality}
\label{sect: extremality}

Note that on $N' \cap M$ the traces coming from $N'$ and from $M$ are
not equal or even comparable, $\pi(N)'$ being a type $\IIinf$ factor
for any representation $\pi$ of $M$, while $M$ is a $\IIone$ factor.
This phenomenon continues up through the tower on all $\M{2i-1}{2i}$.

In the finite index case irreducibility ($N' \cap M=\mathbb{C}$)
implies extremality.  The example constructed by Izumi, Longo and Popa
in~\cite{IzumiLongoPopa1998} shows that this is not true for infinite
index inclusions.  They construct an irreducible $\IIone$ subfactor of
infinite index where the two traces on $N' \cap M_1$ are not even
comparable.

All of this suggests that we should be looking only at $N' \cap
M_{2i+1}$ when defining extremality for general $\IIone$ inclusions.
In this section we give the first definition of extremality in the
infinite index case and show that this definition has as many of the
desired properties as we can expect.

\begin{definition}[Commutant Traces]
Let $r=0,1$.  On $N' \cap M_{2i+r}$ define a trace
$\Trace'_{2i+r}$ by
\[
\Trace'_{2i+r}(x)=\Trace_{2i+1}(J_i x^*J_i) .
\]
In general, on $M_j'\cap M_{2i+r}$ define a trace
$\Trace'_{j,2i+r}$ by
\[
\Trace'_{j,2i+r}(x)=\Trace_{2i-j}(J_i x^*J_i) .
\]
\end{definition}

\begin{remark}
Note that the traces defined above are simply those coming from
representing $M_j$ on $\Ltwo(M_i)$ and using the fact that $J_i M_j'
J_i = M_{2i-j}$ by the multi-step basic construction.  Note that by
Corollary~\ref{cor: traces consistent} $\Trace'_{2i+r}$ is the
canonical trace on $N' \cap \B(\Ltwo(M_i))$.

Finally note that $\Trace'_{2i+1}\br{e_1\cdots e_{2i+1}}=1$.  This is
a consequence of the fact that $\Trace_{2i+1}\br{e_1\cdots
e_{2i+1}}=1$ and $J_i e_1\cdots e_{2i+1} J_i=e_1\cdots e_{2i+1}$:
\begin{align*}
&J_i \pi^{2i+1}_i\br{e_1\cdots e_{2i+1}} J_i 
 \hatr{a_1 \tensorN \cdots \tensorN a_{i+1}} \\
&= J_i \pi^{2i+1}_i\br{1 \tensorN \cdots \tensorN 1}
 \hatr{a_{i+1}^* \tensorN \cdots \tensorN a_1^*} \\
&= J_i \hatr{1 \tensorN \cdots \tensorN 1 
 E_N\br{\cdots E_N\br{E_N\br{a_{i+1}^*}a_i^*}\cdots a_1^*}} \\
&= J_i \hatr{1 \tensorN \cdots \tensorN 1 
 E_N\br{a_{i+1}^*}E_N\br{a_i^*}\cdots E_N\br{a_1^*}} \\
&= \hatr{1 \tensorN \cdots \tensorN 1 
 E_N\br{a_1}\cdots E_N\br{a_{1+1}}} \\
&=\pi^{2i+1}_i\br{e_1\cdots e_{2i+1}}
 \hatr{a_1 \tensorN \cdots \tensorN a_{i+1}}
\end{align*}
Hence we could define $\Trace'_{2i+r}$ as the restriction of the
unique trace on $N'\cap\mathcal{B}(\Ltwo(M_i))$ scaled so that
$\Trace'_{2i+1}(e_1e_3\cdots e_{2i+1})=1$.
\end{remark}

\begin{definition}[Extremality]
Let $N \subset M$ be an inclusion of $\IIone$ factors.  $N \subset M$
is {\em extremal} if $\Trace'_1=\Trace_1$ on $N' \cap M_1$.  $N
\subset M$ is {\em approximately extremal} if $\Trace'_1$ and
$\Trace_1$ are equivalent on $N' \cap M_1$ (i.e. there exists $C>0$
such that $C^{-1} \Trace_1 \leq \Trace'_1 \leq C \Trace_1$ on $N' \cap
M_1$).
\end{definition}

\begin{remark}
We will abuse notation a little by writing
$\Trace'_{2j+1}=\Trace_{2j+1}$ when $\Trace'_{2j+1}=\Trace_{2j+1}$ on
$N' \cap M_{2j+1}$ and similarly $\Trace'_{2j+1}\sim \Trace_{2j+1}$
when $\Trace'_{2j+1}$ and $\Trace_{2j+1}$ are equivalent on $N' \cap
M_{2j+1}$.
\end{remark}

\begin{prop}
\label{prop: equiv defs of extremal}
\begin{description}
\item{(i)} If $N \subset M$ is extremal then
$\Trace'_{2i+1}=\Trace_{2i+1}$ for all $i \geq 0$.
\item{(ii)} If $N \subset M$ is approximately extremal then
$\Trace'_{2i+1}\sim \Trace_{2i+1}$ for all $i \geq 0$.
\item{(iii)} If $\Trace'_{2i+1}=\Trace_{2i+1}$ for some $i \geq 0$
then $N \subset M$ is extremal.
\item{(iv)} If $\Trace'_{2i+1}\sim \Trace_{2i+1}$ for some $i \geq 0$
then $N \subset M$ is approximately extremal.
\end{description}
\end{prop}

\begin{lemma}
\label{lem: Trace' consistent}
For $z\in \plushat{\br{N' \cap M_j}}$,
$T^{N'}_{M_j'}(z)=\Trace'_j(z)1$.
\begin{proof}
Assume $z\in\br{N' \cap M_j}_+$ (in general take $z_k\nearrow z$,
$z_k\in\br{N' \cap M_j}_+$).  $T^{N'}_{M_j'}(z)\in \plushat{M_j' \cap
M_j} = [0,\infty]1$, so $T^{N'}_{M_j'}(z)=\lambda 1$ for some
$\lambda\in[0,\infty]$.  Let $i$ be an integer such that $j=2i$ or
$2i-1$.  Let $\Trace'$ be the canonical trace on $M_j' \cap
\B(\Ltwo(M_i))$.  By Corollary~\ref{cor: traces consistent}
$\Trace'\br{J_i\br{\spdot}^*J_i}=\Trace_{2i-j}=\trace$ and hence
$\Trace'(1)=1$.  Thus
\[
\lambda
=\Trace'\br{T^{N'}_{M_j'}(z)}
=\Trace_{N' \cap \B(\Ltwo(M_i))}(z)
=\Trace'_j(z) .
\]
\end{proof}
\end{lemma}

\begin{lemma}
\label{lem: stepping up and down traces}
\begin{description}
\item
\item{(i)} $\Trace_{2i-1}(x)=\Trace_{2i+1}(xe_{2i+1})$ for $x\in
\plushat{\br{M_{2i-1}}}$.
\item{(ii)} $\Trace_{2i}(x)=\Trace_{2i+1}(e_{2i+1}xe_{2i+1})$ for
$x\in \plushat{\br{M_{2i}}}$.
\item{(iii)} $\Trace'_{2i-1}(x)=\Trace'_{2i+1}\br{xe_{2i+1}}$ for
$x\in \plushat{\br{N' \cap M_{2i-1}}}$.
\end{description}
\begin{proof}
\begin{description}
\item
\item{(i)} $\Trace_{2i+1}(\spdot e_{2i+1})$ is tracial on $M_{2i}$ and
hence a multiple of $\Trace_{2i-1}$.  The multiple is $1$ because
$\Trace_{2i-1}(e_1\cdots e_{2i-1})=1 =\Trace_{2i+1}(e_1\cdots
e_{2i-1}e_{2i+1})$.
\item{(ii)} $e_{2i+1}xe_{2i+1}=E_{M_{2i-1}}(x)e_{2i+1}$ so by (i)
\[
\Trace_{2i+1}\br{e_{2i+1}xe_{2i+1}}
=\Trace_{2i-1}\br{E_{M_{2i-1}}(x)}
=\Trace_{2i}\br{x} .
\]
\item{(iii)} First note that
$T^{M_{2i-1}'}_{M_{2i+1}'}\br{ e_{2i+1}}=1$: take a basis $\{ b_j \}$
for $M_{2i}$ over $M_{2i-1}$.  Then $\{ b_j e_{2i+1} b_k \}$ is a
basis for $M_{2i+1}$ over $M_{2i-1}$ and hence
\[
T^{M_{2i-1}'}_{M_{2i+1}'}\br{ e_{2i+1}}
= \sum_{j,k} b_j e_{2i+1} b_k e_{2i+1} b_k^* e_{2i+1} b_j^* 
= \sum_j b_j e_{2i+1} b_j^* = 1 .
\]

Let $x \in (N' \cap M_{2i-1})_+$.  Using Lemma~\ref{lem: Trace'
consistent}
\begin{align*}
\Trace'_{2i+1}\br{xe_{2i+1}} 1
&= T^{N'}_{M_{2i+1}'}\br{ xe_{2i+1} }  \\
&= T^{M_{2i-1}'}_{M_{2i+1}'}\br{ T^{N'}_{M_{2k-1}'}
     \br{ xe_{2i+1}}} \\
&= T^{M_{2i-1}'}_{M_{2i+1}'}\br{ T^{N'}_{M_{2i-1}'}(x) e_{2i+1}} \\
&= T^{M_{2i-1}'}_{M_{2i+1}'}\br{ \Trace'_{2i-1}(x) e_{2i+1}} \\
&= \Trace'_{2i-1}(x) T^{M_{2i-1}'}_{M_{2i+1}'}\br{ e_{2i+1}} \\
&= \Trace'_{2i-1}(x) 1 .
\end{align*}
\end{description}
\end{proof}
\end{lemma}


\Proof {\it of Prop~\ref{prop: equiv defs of extremal}.}

In the finite index case the proof is easily accomplished using planar
algebra machinery.  $\Trace_{2i+1}$ is just closing up a $2i+2$-box on
the right, $\Trace'_{2i+1}$ is closing up a $2i+2$-box on the left.
Extremality means that a $2$-box closed on the left is equal to the
same box closed on the right.  For a $2i+2$-box just move the strings
from right to left two at a time.  This is the approach that we will
take here, although of course we cannot use the planar algebra
machinery and must proceed algebraically.

\begin{description}
\item{(i)} Suppose $\Trace_{2i-1}=\Trace'_{2i-1}$.  We will show that
$\Trace_{2i+1}=\Trace'_{2i+1}$.  Let $z \in \br{N' \cap M_{2i+1}}_+$,
then,
\begin{align*}
&\Trace_{2i+1}(z) 1 \\
&=\Trace_{2i-1} \br{T_{M_{2i-1}}(z)} 1 \\
&=\Trace'_{2i-1} \br{T_{M_{2i-1}}(z)} 1 \\
&=T^{N'}_{M_{2i-1}'} \br{T_{M_{2i-1}}(z)}
  &\text{by Lemma~\ref{lem: Trace' consistent}} \\
&=\sum_b b T_{M_{2i-1}}(z) b^*
  &\text{where $\{ b \}$ is a basis for $M_{2i-1}$ over $N$} \\
&=\sum_b T_{M_{2i-1}}(bzb^*) \\
&=T_{M_{2i-1}}\br{T^{N'}_{M_{2i-1}'}(z)} 
  &\text{now represent everything on }\Ltwo(M_i) \\
&=j_i T^{N'}_{M_1'}\br{j_i\br{T^{N'}_{M_{2i-1}'}(z)}}
  &\text{because }j_i\br{M'_{2i-1}\cap M_{2i+1}}=M_1 \cap N' \\
&=\Trace'_1\br{j_i\br{T^{N'}_{M_{2i-1}'}(z)}}1 
  &\text{by Lemma~\ref{lem: Trace' consistent}} \\
&=\Trace_1\br{j_i\br{T^{N'}_{M_{2i-1}'}(z)}}1 \\
&=\Trace_{M_{2i-1}'\cap \B(\Ltwo(M_i))}\br{T^{N'}_{M_{2i-1}'}(z)}1 \\
&=\Trace_{N'\cap \B(\Ltwo(M_i))}(z)1 \\
&=\Trace'_{2i+1}(z)1
\end{align*}

\item{(iii)} Suppose $\Trace_{2i+1}=\Trace'_{2i+1}$, $i \geq 1$.
Using Lemma~\ref{lem: stepping up and down traces}, for $z \in \br{N'
\cap M_{2i-1}}_+$,
\[
\Trace_{2i-1}(z)
=\Trace_{2i+1}(ze_{2i+1})
=\Trace'_{2i+1}(ze_{2i+1})
=\Trace'_{2i-1}(z) .
\]

\item{(ii) and (iv)} Similar to (i) and (iii) with inequalities and
constants.

\end{description}
\proofend


==> inf/finiteindexrecall.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FINITE INDEX
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Finite Index Recollections}
\label{sect: finite index IIone}

Here we recall some results on finite index subfactors.

\begin{definition}[Extremal]
A finite index $\IIone$ subfactor $N \subset M$ is called {\em
extremal} if the unique traces $\trace'_0$ and $\trace_0$ on $N'$ and
$M$ respectively coincide on $N' \cap M$ (where $N'$ is calculated on
any Hilbert space on which $M$ acts with finite $M$-dimension).  We
will write this as $\trace'_0=\trace_0$.
\end{definition}

\begin{remark}
Note that in particular an irreducible finite index $\IIone$ subfactor
($N' \cap M = {\mathbb C}$) is extremal.  In~\cite{PimsnerPopa1986}
and~\cite{PimsnerPopa1988} Pimsner and Popa show that extremality is
equivalent to the condition that $\trace'_i=\trace_i$ for some $i \geq
0$ or for any $i \geq 0$.
\end{remark}

\subsection{Rotations}

Let $N \subset M$ be a finite index $\IIone$ subfactor.  We use the
following notations: $\delta=[M:N]^{1/2}$, $E_k=\delta e_k$, $v_k=E_k
E_{k-1} \cdots E_1$.  $B=\{ b \} = \{ b_i \}$ denotes a basis for $M$
over $N$ (i.e. $\sum_b b e_1 b^* =1$).

On $N' \cap M_k$ define the rotation $\rho_k$ by
\begin{align*}
\rho_k(x)
&=\delta^2 E_{M_k}(v_{k+1}E_{M'}(x v_{k+1})) \\
&=\sum_{b \in B}
  \sum_i E_N\br{bx^{(i)}_1}x^{(i)}_2\tensorN x^{(i)}_3 \tensorN 
          \cdots \tensorN x^{(i)}_{k+1} \tensorN b^*
\end{align*}
where $x=\sum_i x^{(i)}_1 \tensorN x^{(i)}_2 \tensorN \cdots \tensorN
x^{(i)}_{k+1}$.  The equality of the two expressions for $\rho_k(x)$
is proved using exactly the same argument as in Lemma 4.1.14
of~\cite{Jones1999}.  $E_{M'}=\tau \sum b \spdot b^*$ is still true in
the nonextremal case, see Proposition 2.7 of~\cite{Bisch1995}.

Define the operator $\wtilde{\rho}_k$ on basic tensors $x=x_1 \tensorN
x_2 \tensorN \cdots \tensorN x_{k+1}$ in $M_k$ by
\[
\wtilde{\rho}_k(x)
=P_c \br{x_2 \tensorN x_3 \tensorN \cdots \tensorN x_{k+1} \tensorN x_1},
\]
where $P_c$ is the orthogonal projection onto the $N$-central vectors
in $\Ltwo(M_k,\trace)$, which is just the finite dimensional subspace
$N' \cap M_k$.  $P_c$ above could thus be replaced by $E_{N' \cap
M_k}$, the unique trace-preserving conditional expectation from
$(M_k,\trace)$ to $(N' \cap M_k,\trace)$.  $\wtilde{\rho}_k$ is
extended to all of $M_k$ by linearity.

\begin{remark}
In~\cite{Jones1999} Jones shows that in the extremal case
$\rho=\wtilde{\rho}$ and periodicity of $\rho$ follows from that of
$\wtilde{\rho}$.  In the nonextremal case H. P. Huang shows
in~\cite{Huang2000} that $\rho$ and $\wtilde{\rho}$ are periodic.
\end{remark}

\begin{prop}
\label{prop: rho inner product}
For all $x \in N' \cap M_k$ and for all $y_i \in M$,
\[
\ip{\rho_k(x), y_1 \tensorN y_2 \tensorN \cdots \tensorN y_{k+1}}
=\ip{x, y_{k+1} \tensorN y_1 \tensorN \cdots \tensorN y_k}
\]
where the inner product is that on $\Ltwo(M_k,\trace)$.
\end{prop}

\begin{cor}
$\br{\rho_k}^{k+1}=\id$ and on $\Ltwo(N' \cap M_k,\trace)$
$\wtilde{\rho}_k=\br{\rho_k^{-1}}^*$ (and hence
$\br{\wtilde{\rho}_k}^{k+1}=\id$).
\end{cor}

\begin{cor}
\label{cor: rho to tilde rho via RN}
For $y \in N' \cap M_k$,
$\wtilde{\rho}_k(y)=\rho_k(y)z_1=\rho_k(z_1^{-1}y)$ where $z_1$ is the
Radon-Nikodym derivative of $\trace'_1$ with respect to $\trace_1$ on
$N' \cap M_1$ (i.e. $\trace'_1(x)=\trace(z_1x)$ for all $x\in N'\cap
M_1$).
\begin{proof}
Let $x \in N' \cap M_k$.  Note from Prop~\ref{prop: rho inner product}
that $(\rho_k(x^*))^*=\rho_k^{-1}(x)$: Let $y= y_1 \tensorlN \cdots
\tensorlN y_{k+1}$, then
\begin{align*}
\ip{\rho_k(x^*)^*,y}
&=\ip{y_{k+1}^* \tensorN y_k^* \tensorN \cdots \tensorN y_1^*,
  \rho_k(x^*)} \\
&=\ip{y_1^* \tensorN y_{k+1}^* \tensorN \cdots \tensorN y_2^*,
  x^*} \\
&=\ip{x,
  y_2 \tensorN \cdots \tensorN y_{k+1} \tensorN y_1 } \\
&=\ip{\rho_k^{-1}(x),y} .
\end{align*}
\newpage
Let $y \in N' \cap M_k$.  Then, writing a thick string to represent
$k-1$ regular strings,
\begin{align*}
&\delta^{k+1}\trace(x^* \wtilde{\rho}_k(y))
= \delta^{k+1}\ip{\wtilde{\rho}_k(y),x}
= \delta^{k+1}\ip{y,\rho_k^{-1}(x)}
= \delta^{k+1}\ip{y,(\rho_k(x^*))^*} \\
& \phantom{\delta^{k+1}}= \delta^{k+1}\trace(\rho_k(x^*)y) \\
\end{align*}
\vspace{-10mm}
\begin{figure}[htbp]
\begin{center}
\psfrag{y}{$y$}
\psfrag{x^*}{$x^*$}
\psfrag{=}{$=$}
\psfrag{z_1}{$z_1$}
\psfrag{z_1^-1}{$z_1^{-1}$}
\includegraphics{fig/rho_rhotilde.eps}
%\caption{The caption on your figure}
%\label{figure:yourreferencename}
\end{center}
\end{figure}
\vspace{-5mm}
\begin{align*}
&\hspace{-10mm} = \delta^{k+1} \trace(x^* \rho_k(y) z_1) 
&=\delta^{k+1} \trace(x^* \rho_k(z_1^{-1} y))
\end{align*}
Hence $\wtilde{\rho}_k(y)=\rho_k(y) z_1=\rho_k(z_1^{-1} y)$.
\end{proof}
\end{cor}

\begin{remark}
It is also possible to prove Corollary~\ref{cor: rho to tilde rho via
RN} by starting with the second definition of $\rho$ and averaging
over the unitary group of $N$ ($\{ ub \}$ is still a basis if $u \in
\mathcal{U}(N)$).  This technique, a frequent tool of Popa first found
in~\cite{Popa1981}, leads one to considering $E_{N' \cap M_1}(\sum
b^*e_1b)=z_1$.
\end{remark}

\newpage
\Proof {\it of Prop~\ref{prop: rho inner product}.}

For $a \in M$ define operators $L_a, R_a:\Ltwo(M_{k-1},\trace)
\rightarrow \Ltwo(M_k,\trace)$ by $L_a \xi=\hatt{a} \tensorlN \xi$ and
$R_a \xi = \xi \tensorlN \hatt{a}$.  Note that $\br{L_a}^*
\hatt{b} \tensorlN \eta = E_N(a^*b)\eta$:
\begin{align*}
\ip{\br{L_a}^* \hatt{b} \tensorN \eta,\xi}
&=\ip{\hatt{b} \tensorN \eta, \hatt{a} \tensorN \xi} \\
&=\ip{\ip{\hatt{a},\hatt{b}}_N \eta, \xi} \\
&=\ip{E_N(a^*b) \eta, \xi} .
\end{align*}
By a similar argument, or using $R_a=J_k L_{a^*} J_{k-1}$, $\br{R_a}^*
\eta \tensorlN \hatt{b}= \eta E_N(ba^*)$.  Hence:
\begin{align*}
\rho_k(x)
&=\sum_{b \in B}
  \sum_i E_N\br{bx^{(i)}_1}x^{(i)}_2\tensorN x^{(i)}_3 \tensorN 
  \cdots \tensorN x^{(i)}_{k+1} \tensorN b^* \\
&=\sum_{b \in B}
  R_{b^*} \br{ L_{b^*}}^* x .
\end{align*}
Finally
\begin{align*}
\ip{\rho_k(x),y}
&=\sum_b \ip{x, L_{b^*} \br{ R_{b^*}}^* y} \\
&=\sum_b \ip{x, b^* \tensorN y_1 \tensorN \cdots \tensorN y_k E_N(y_{k+1}b)} \\
&=\sum_b \ip{xE_N(y_{k+1}b)^*,b^* \tensorN y_1 \tensorN \cdots \tensorN y_k} \\
&=\sum_b \ip{E_N(y_{k+1}b)^*x,b^* \tensorN y_1 \tensorN \cdots \tensorN y_k} \\
&=\sum_b \ip{x,E_N(y_{k+1}b)b^* \tensorN y_1 \tensorN \cdots \tensorN y_k} \\
&= \ip{x,y_{k+1} \tensorN y_1 \tensorN \cdots \tensorN y_k}
\end{align*}
\proofend


==> inf/rotandextremality.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ROTATIONS AND EXTREMALITY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Rotations and Extremality}
\label{sect: rotations and extremality}

We prove that approximate extremality is necessary and sufficient for
the rotations to exist.

\begin{prop}
\label{prop: approx extremal implies rotation}
\begin{description}
\item{}
\item{(i)} If $N \subset M$ is approximately extremal then $\rho^B_k$
exists for all bases $B$ and for all $k \geq 0$.  In this case we will
use the notation $\rho_k$.
\item{(ii)} If $N \subset M$ is extremal then in addition to (i)
$\rho_k$ is a unitary operator on $N' \cap \Ltwo(M_k)$.  Hence
$\rho_k=\wtilde{\rho}_k$.
\end{description}
\end{prop}

\begin{lemma}
\label{lem: stuff about e_1}
\begin{description}
\item
\item{(i)} $L_1 \br{L_1}^*=e_1$.
\item{(ii)} $J_ie_1 J_i=e_{2i+1}$.
\item{(iii)} For $x\in \br{M' \cap M_k}_+$,
$e_1xe_1=T^{M'}_{M_1'}(x)e_1$.
\end{description}
\begin{proof}
\begin{description}
\item{(i)} With the usual notations established in the proof of
Prop~\ref{prop: tensorP},
\begin{align}
e_1 \hatr{a_1 \tensorN \cdots \tensorN a_{i+1}}
&= e_1 \hatr{A_1 \tensorM \cdots \tensorM \overline{A}_i} \nonumber \\
&= \hatr{\br{e_1A_1} \tensorM \cdots \tensorM \overline{A}_i} \nonumber \\
&= \hatr{\br{E_N(a_1)e_1w_1} \tensorM A_2 \tensorM \cdots 
   \tensorM \overline{A}_i} \nonumber \\
&= \hatr{E_N(a_1) \tensorN a_2 \tensorN \cdots \tensorN a_{i+1}} 
   \label{eq: e_1 action} \\
&= L_1 \hatr{E_N(a_1)a_2 \tensorN a_3 \tensorN \cdots \tensorN a_{i+1}} 
   \nonumber \\
&= L_1 \br{L_1^*L_{a_1}}\hatr{a_2 \tensorN a_3 \tensorN \cdots \tensorN 
   a_{i+1}} \nonumber \\
&= L_1L_1^* \hatr{a_1 \tensorN a_2 \tensorN \cdots \tensorN a_{i+1}} \nonumber .
\end{align}
\item{(ii)} From (\ref{eq: e_1 action}), $J_ie_1J_i\hatr{a_1 \tensorlN
\cdots \tensorlN a_{i+1}}=\hatr{a_1 \tensorlN \cdots \tensorlN a_i
\tensorlN E_N(a_{i+1})}$.  Let $\iota:\Ltwo(M_{2i-1})\rightarrow
\Ltwo(M_{2i})$ be the inclusion map.  From the definition of
$\pi^{2i+1}_i$,
\begin{align*}
&\sqbr{\pi^{2i+1}_i\br{e_{2i+1}}\hatr{a_1 \tensorN \cdots \tensorN a_{i+1}}} 
  \tensorN \hatr{b_1 \tensorN \cdots \tensorN b_i} \\
&=e_{2i+1} \hatr{a_1 \tensorN \cdots \tensorN a_{i+1}
  \tensorN b_1 \tensorN \cdots \tensorN b_i} \\
&=\iota \hatr{E_{M_{2i-1}}\br{a_1 \tensorN \cdots \tensorN a_{i+1}
  \tensorN b_1 \tensorN \cdots \tensorN b_i}} \\
&=\iota \hatr{a_1 \tensorN \cdots \tensorN a_iE_N(a_{i+1})
  \tensorN b_1 \tensorN \cdots \tensorN b_i} \\
&=\hatr{a_1 \tensorN \cdots \tensorN a_iE_N(a_{i+1}) \tensorN 1
  \tensorN b_1 \tensorN \cdots \tensorN b_i} \\
&=\sqbr{e_1\hatr{a_1 \tensorN \cdots \tensorN a_{i+1}}} 
  \tensorN \hatr{b_1 \tensorN \cdots \tensorN b_i} .
\end{align*}
\item{(iii)} For $x\in \br{M' \cap M_k}_+$,
\[
e_1xe_1
=J_ie_{2i+1} J_ixJ_i e_{2i+1}J_i
=J_i E_{M_{2i-1}}\br{J_ixJ_i}e_{2i+1} J_i
=T^{M'}_{M_1'}(x) e_1 .
\]
\end{description}
\end{proof}
\end{lemma}

\Proof {\it of Prop~\ref{prop: approx extremal implies rotation}.}
\begin{description}
\item{(i)} First consider $k=2l+1$.  Then, for $x \in N' \cap
\gothn_{\Trace_k}$,
\begin{align*}
\left|\left| \sum_{i=r}^s R_{b_i^*} \br{ L_{b_i^*} }^* x \right|\right|^2
&= \sum_{i=r}^s \sum_{j=r}^s
	\ip{ \br{R_{b_j^*}}^* R_{b_i^*} \br{L_{b_i^*}}^*x,
	  \br{L_{b_j^*}}^*x } \\
&= \sum_{i=r}^s \sum_{j=r}^s
	\ip{ \br{\br{L_{b_i^*}}^*x}\cdot E_N(b_i^*b_j),
	  \br{L_{b_j^*}}^*x } \\
&\leq \sum_{i=r}^s
	\ip{ \br{L_{b_i^*}}^*x,
	  \br{L_{b_j^*}}^*x } ,
\end{align*}
because $[E_N(b_i^* b_j)]_{i,j=r, \ldots, s} \in M_{s-r+1}(N)$ is
dominated by $1=\delta_{i,j}$ (basically because the infinite matrix
$[E_N(b_i^* b_j)]$ is a projection).  Hence
\begin{align*}
\left|\left| \sum_{i=r}^s R_{b_i^*} \br{ L_{b_i^*} }^* x \right|\right|^2
&\leq \sum_{i=r}^s ||\br{L_{b_i^*}}^*x ||^2 \\
&=    \sum_{i=r}^s ||\br{b_i^* L_1}^*x ||^2 \\
&=    \sum_{i=r}^s \ip{ L_1\br{L_1}^* b_i x, b_i x } \\
&=    \sum_{i=r}^s \ip{ e_1 b_i x, b_i x } 
      &\text{by Lemma~\ref{lem: stuff about e_1}} \\
&=    \sum_{i=r}^s \Trace_k\br{ e_1 b_i xx^* b_i^* e_1 } .
\end{align*}
$\sum_{i=1}^s b_i xx^* b_i^* \nearrow T^{N'}_{M'}(xx^*)$ and hence
$\sum_{i=1}^s e_1 b_i xx^* b_i^* e_1 \nearrow
E^{M'}_{M_1'}\br{T^{N'}_{M'}(xx^*)} e_1$, by Lemma~\ref{lem: stuff
about e_1}.  Thus,
\begin{align}
\sum_{i=1}^s \Trace_k\br{ e_1 b_i xx^* b_i^* e_1 }
&\nearrow \Trace_k\br{ e_1 T^{N'}_{M_1'}(xx^*) } \nonumber \\
&\leq C \Trace'_k\br{ e_1 T^{N'}_{M_1'}(xx^*) } \nonumber \\
&= C\Trace_{2l+1}\br{j_l\br{e_1 T^{N'}_{M_1'}(xx^*)}} \nonumber \\
&= C\Trace_{2l+1}\br{j_l\br{T^{N'}_{M_1'}(xx^*)}e_{2l+1}} 
   &\text{by Lemma~\ref{lem: stuff about e_1}} \nonumber \\
&= C\Trace_{2l-1}\br{j_l\br{T^{N'}_{M_1'}(xx^*)}} 
   &\text{by Lemma~\ref{lem: stepping up and down traces}} \nonumber \\
&= C\Trace_{M_1'\cap\B(\Ltwo(M_l))}\br{T^{N'}_{M_1'}(xx^*)}
   &\text{by Corollary~\ref{cor: traces consistent}} \nonumber \\
&= C\Trace_{N'\cap\B(\Ltwo(M_l))}(xx^*) \nonumber \\
&= C \Trace'_k(xx^*) \nonumber \\
&\leq C^2 \Trace_k(xx^*) \nonumber \\
&= C^2 ||x||_2^2 . \label{eq: rotn existence 1}
\end{align}
Hence $\sum_{i=r}^s \Trace_k\br{ e_1 b_i xx^* b_i^* e_1 } \rightarrow
0$ and so $\{ \sum_{i=1}^s R_{b_i^*} \br{ L_{b_i^*} }^* \hatt{x} \}$
is Cauchy and hence converges.  In addition $||\sum_{i=1}^\infty
R_{b_i^*} \br{ L_{b_i^*} }^* \hatt{x}|| \leq C||\hatt{x}||$, so that
$\rho^B_k$ exists and $||\rho^B_k|| \leq C$.

\vspace{4mm}

For $k=2l$ we begin as above. For $x \in N' \cap \gothn_{\Trace_k}$,
\[
\left|\left| \sum_{i=r}^s R_{b_i^*} \br{ L_{b_i^*} }^* x \right|\right|^2
\leq \sum_{i=r}^s \Trace_k\br{ e_1 b_i xx^* b_i^* e_1 } .
\]
By (\ref{eq: rotn existence 1}) and Lemma~\ref{lem: stepping up and
down traces},
\begin{align*}
\sum_{i=1}^s \Trace_k\br{ e_1 b_i xx^* b_i^* e_1 }
&= \sum_{i=1}^s \Trace_k\br{ e_1 b_i x e_{2l+1} x^* b_i^* e_1 } \\
&\leq C^2 \Trace_{2l+1}\br{ e_{2l+1}xx^*e_{2l+1} } \\
&= C^2 \Trace_{2l}(xx^*) ,
\end{align*}
and the remainder of the argument proceeds exactly as in the $k=2l+1$
case.

\item{(ii)} If $N \subset M$ is extremal then $C=1$ so that
$||\rho_k||\leq 1$.  As $\rho_k$ is periodic this implies that
$\rho_k$ is a unitary operator.
\end{description}
\proofend


In order to establish the converse result we connect $\rho_k$ to
$J\spdot J$.

\begin{prop}
\label{prop: rotn implies 1/2 turn = Jx^*J}
\begin{description}
\item{}
\item{(i)} If either $\rho^B_{2k-1}$ exists or $\rho^B_{2k}$ exists then
$\sigma: \Ltwo(M_{2k-1}) \rightarrow N' \cap \Ltwo(M_{2k-1})$ defined by
\[
y_1 \tensorN \cdots \tensorN y_{2k} \mapsto
 P_c\br{ y_{k+1} \tensorN y_{k+2} \tensorN \cdots \tensorN y_{2k}
           \tensorN y_1 \tensorN y_2 \tensorN \cdots \tensorN y_k } ,
\]
exists (extends to a bounded operator, also denoted $\sigma$).
\item{(ii)} In that case let $\mu=\br{ \sigma |_{N' \cap
\Ltwo(M_{2k-1})} }^*$.  Then $\mu\br{ N' \cap
\gothn_{\Trace_{2k-1}} } = N' \cap \gothn_{\Trace_{2k-1}}$ and
\begin{align*}
&\mu(x)= J_{k-1} x^* J_{k-1}
& \text{for } x \in N' \cap \gothn_{\Trace_{2k-1}}
\end{align*}
\end{description}
\begin{proof}

\begin{description}
\item
\item{(i)} If $\rho^B_{2k-1}$ exists then by (\ref{eq: rho inner
prod}) in the proof of Theorem~\ref{thm: rho, tilde(rho)},
$\sigma=\br{ \rho_{2k-1}^k \circ P_c }^*$.  If $\rho_{2k}$ exists
then, for $x \in N' \cap \gothn_{\Trace_{2k-1}}$ and $y=\sum_i
y_1^{(i)} \tensorlN \cdots \tensorlN y_{2k}^{(i)}$,
\begin{align*}
&\ip{x, \sum_i P_c \br{ y_{k+1}^{(i)} \tensorN \cdots \tensorN
             y_{2k}^{(i)} \tensorN y_1^{(i)} \tensorN \cdots \tensorN
             y_k^{(i)} } }_{\Ltwo(M_{2k-1})} \\
&=\ip{x,\sum_i y_{k+1}^{(i)} \tensorN \cdots \tensorN
             y_{2k}^{(i)} \tensorN y_1^{(i)} \tensorN \cdots \tensorN
             y_k^{(i)} }_{\Ltwo(M_{2k-1})} \\
&=\ip{x,\sum_i y_{k+1}^{(i)} \tensorN \cdots \tensorN
             y_{2k}^{(i)} \tensorN y_1^{(i)} \tensorN \cdots \tensorN
             y_k^{(i)} }_{\Ltwo(M_{2k})} \\
&=\ip{x,\sum_i y_{k+1}^{(i)} \tensorN \cdots \tensorN y_{2k}^{(i)} \tensorN 
             1 \tensorN y_1^{(i)} \tensorN \cdots \tensorN
             y_k^{(i)} }_{\Ltwo(M_{2k})} \\
&=\ip{\rho_{2k}^k(x), \sum_i 1 \tensorN y_1^{(i)} \tensorN \cdots \tensorN 
             y_{2k}^{(i)} } \\
&=\ip{\br{ L_1}^* \rho_{2k}^k(x), y} .
\end{align*}
Letting $z=\sum_i P_c \br{ y_{k+1}^{(i)} \tensorN \cdots \tensorN
             y_{2k}^{(i)} \tensorN y_1^{(i)} \tensorN \cdots \tensorN
             y_k^{(i)} }$,
\begin{align*}
|| z ||_2
&=\sup \{ |<x,z>| : x \in N' \cap \Ltwo(M_{2k-1}), ||x||_2=1 \} \\
&\leq \left|\left| \br{ L_1}^* \rho_{2k}^k \right|\right| ||y||_2 \\
&\leq \left|\left|\rho_{2k}\right|\right|^k ||y||_2 .
\end{align*}
Hence $\sigma$ exists.

\item{(ii)} We proceed in four steps:
\begin{description}
\item{(1)} For $y \in \gothn_{\Trace_{2k-1}}$ and for $\xi, \eta \in
\Ltwo(M_{k-1})$ satisfying either $\xi \in D(\Ltwo(M_{k-1})_N)$ or
$\eta \in D(\Ltwo(M_{k-1})_N)$, we have
\[
\ip{\hatt{y}, \xi \tensorN J_{k-1} \eta }_{\Ltwo(M_{2k-1})}
=\ip{y \eta, \xi }_{\Ltwo(M_{k-1})} .
\]
This is easily established by first taking both $\xi, \eta \in
D(\Ltwo(M_{k-1})_N)$, and the general result then follows by
continuity.  Using Lemma~\ref{lemma: Trace = norm},
\begin{align*}
\ip{ \hatt{y} , \xi \tensorN J_{k-1} \eta }_{\Ltwo(M_{2k-1})}
&= \ip{ y , L(\xi)L(\eta)^* }_{\Ltwo(M_{2k-1})} \\
&= \Trace_{2k-1}\br{y L(\eta) L(\xi)^* } \\
&= \Trace_{2k-1}\br{L(y\eta) L(\xi)^* } \\
&= \ip{y \eta, \xi} .
\end{align*}

\item{(2)} For $y \in N' \cap \gothn_{\Trace_{2k-1}}$ satisfying
$J_{k-1} y^* J_{k-1} \in \gothn_{\Trace_{2k-1}}$ we have
\[
\mu(\hatt{y}) = J_{k-1} y^* J_{k-1} .
\]
To prove this first note that for $\xi \in N' \cap \Ltwo(M_{2k-1})$
and $\eta, \zeta \in D(\Ltwo(M_{k-1})_N)$ or $\eta, \zeta \in
D(\leftidx{_N}{\Ltwo(M_{k-1})})$,
\[
\ip{ \mu(\xi) , \eta \tensorN \zeta }
= \ip{ \xi , \zeta \tensorN \eta } .
\]
The result is true for $\eta=\hatt{a}$, $\zeta=\hatt{b}$, where $a, b
\in \wtilde{M}_{k-1}$ and the general result follows by density.

Now, using the result from (1),
\begin{align*}
\ip{ J_{k-1} y^* J_{k-1} , \eta \tensorN \zeta }_{2k-1}
&= \ip{ J_{k-1} y^* J_{k-1} J_{k-1} \zeta , \eta }_{k-1} \\
&= \ip{ J_{k-1} \eta , y^* \zeta }_{k-1} \\
&= \ip{ y J_{k-1} \eta , \zeta }_{k-1} \\
&= \ip{ y , \zeta \tensorN \eta }_{2k-1} \\
&= \ip{ \mu(\hatt{y}) , \eta \tensorN \zeta }_{2k-1} .
\end{align*}
Hence $ J_{k-1} y^* J_{k-1} =\mu(\hatt{y})$.

\item{(3)} Let $p$ be the maximal central projection in $N' \cap
M_{2k-1}$ such that $\Trace_{2k-1}$ is semifinite on $p(N' \cap
M_{2k-1})$.  Let $A=p(N' \cap M_{2k-1})$.  We will show that if $x \in
N' \cap \gothn_{\Trace_{2k-1}}$ then $\xi=\mu(\hatt{x})$ is a bounded
vector in $A$ (i.e. in $D(\Ltwo(A)_A)$) and hence an element of $A$.

Let $a \in N' \cap \gothn_{\Trace_{2k-1}}$ and let $y=J_{k-1}a^*
J_{k-1} x$.  Note that $y$ satisfies the conditions of (2).  Now, with
all supremums taken over $\sum \eta_i \tensorlN \zeta_i$ such that
$\left|\left|\sum \eta_i \tensorlN \zeta_i \right|\right|=1$, we have:
\begin{align*}
|| \xi a ||
&= \sup \left| \ip{ \xi a , \sum \eta_i \tensorN \zeta_i } \right| \\
&= \sup \left| \sum \ip{ \xi , 
     J_{2k-1} a J_{2k-1} \eta_i \tensorN \zeta_i } \right| \\
&= \sup \left| \sum \ip{ \xi , 
     J_{2k-1} \br{a J_{k-1} \zeta_i \tensorN J_{k-1}\eta_i} } \right| \\
&= \sup \left| \sum \ip{ \xi , 
     J_{2k-1} \br{\br{a J_{k-1} \zeta_i} \tensorN J_{k-1}\eta_i} } \right| \\
&= \sup \left| \sum \ip{ \xi , 
     \eta_i \tensorN J_{k-1} a J_{k-1} \zeta_i } \right| \\
&= \sup \left| \sum \ip{ x , 
     J_{k-1} a J_{k-1} \zeta_i \tensorN \eta_i } \right| \\
&= \sup \left| \sum \ip{ J_{k-1} a^* J_{k-1} x , 
      \zeta_i \tensorN \eta_i } \right| \\
&= \sup \left| \sum \ip{ y , 
      \sigma\br{\eta_i \tensorN \zeta_i } } \right| \\
&= \sup \left| \sum \ip{ \mu(y) , 
      \eta_i \tensorN \zeta_i } \right| \\
&= \left|\left| \mu(y) \right|\right|_{\Ltwo(M_{2k-1})} \\
&= \left|\left| J_{k-1} y^* J_{k-1} \right|\right|_2 \\
&= \left|\left| a^* J_{k-1} x J_{k-1} \right|\right|_2 \\
&\leq ||a||_2 ||x|| .
\end{align*}
Hence $\xi$ is a bounded vector and thus an element of $A$.

%% In detail: $\pi_l(\xi) \in \pi_r(A)'=\pi_l(A)$.  Let $\pi_l(\xi)=z \in
%% A$.  Then $\Trace(z^*z)=||\xi||^2<\infty$ and $\xi=\hatt{z}$:
%% \[
%% ||\xi-\hatt{z}||^2
%% =2||z||_2^2-2\mathrm{Re}<\xi,z>=0
%% \]
%% because
%% \[
%% <\xi,z>
%% =\lim <\xi, p_i z>
%% =\lim <\xi z^*, p_i >
%% =\lim <zz^*, p_i>
%% =||z||_2^2.
%% \]

\item{(4)} Finally, let $z \in N' \cap \gothn_{\Trace_{2k-1}}$ such
that $\mu(\hatt{x})=\hatt{z}$.  Then $z=J_{k-1} x^* J_{k-1}$ because
\begin{align*}
\ip{ J_{k-1} x^* J_{k-1} \eta, \zeta }
&= \ip{ x J_{k-1} \zeta , J_{k-1} \eta } \\
&= \ip{ x , J_{k-1} \eta \tensorN \zeta } \\
&= \ip{ \mu(x) , \zeta \tensorN J_{k-1} \eta } \\
&= \ip{ z , \zeta \tensorN J_{k-1} \eta } \\
&= <z \eta , \zeta > .
\end{align*}
\end{description}
\end{description}
\end{proof}
\end{prop}

\begin{prop}
\label{prop: rotn implies approx ext}
\begin{description}
\item{(i)} If $\rho^B_i$ exists then $N \subset M$ is approximately
extremal.
\item{(ii)} If $\rho^B_i$ exists and is a unitary operator then $N
\subset M$ is extremal.
\end{description}
\begin{proof}

\begin{description}
\item{(i)} Let $j$ be the largest odd number with $j \leq i$.  By
Prop~\ref{prop: rotn implies 1/2 turn = Jx^*J} there exists $\mu:N'
\cap \Ltwo(M_j) \rightarrow N' \cap \Ltwo(M_j)$ with $||\mu|| \leq
\left|\left| \rho_i \right|\right|^k$ (where $j=2k-1$) and
$\mu(x)=J_{k-1} x^* J_{k-1}$ for $x \in N' \cap
\gothn_{\Trace_j}$.

We first show that $\Trace'_j \leq ||\mu||^2 \Trace_j$.  Take $x \in
N' \cap M_j$.  If $\Trace_j(x^*x)=\infty$ then we are done.  Otherwise
$x \in \gothn_{\Trace_j}$ and
\begin{align*}
\Trace'_j(x^8x)
&= \Trace_j \br{ J_{k-1} x^* J_{k-1} J_{k-1} x J_{k-1} } \\
&= \Trace_j ( \mu(x) \mu(x)^*) \\
&\leq ||\mu||^2 ||x||_2^2 \\
&= ||\mu||^2 \Trace_j(x^*x) .
\end{align*}

Finally, 
$\Trace_j
=\Trace'_j\br{J_{k-1}\spdot J_{k-1}}
\leq ||\mu||^2 \Trace_j\br{J_{k-1}\spdot J_{k-1}}
= ||\mu||^2 \Trace'_j$.

\item{(ii)} If $\rho_i$ is unitary then $||\mu|| \leq 1$ so that
$\Trace_j \leq \Trace'_j \leq \Trace_j$ and hence $\Trace_j =
\Trace'_j$.
\end{description}
\end{proof}
\end{prop}

\begin{cor}
\label{cor: rotn for one basis implies rotn for all}
If there exists a basis $B$ such that $\rho^B_k$ exists then for any
basis $\overline{B}$, $\rho^{\overline{B}}_k$ exists and is
independent of the basis used.  Hence we will use $\rho_k$ to denote
$\rho^B_k$.
\begin{proof}

Suppose $\rho^B_k$ exists.  By Prop~\ref{prop: rotn implies approx
ext} the subfactor is approximately extremal.  By Prop~\ref{prop:
approx extremal implies rotation} $\rho^{\overline{B}}_k$ exists for
any basis $\overline{B}$.  By Theorem~\ref{thm: rho, tilde(rho)}
$\rho_k$ is independent of the basis used.
\end{proof}
\end{cor}


The results of Sections \ref{sect: extremality} through \ref{sect:
rotations and extremality} can be summarized as follows.

\begin{thm}
\begin{description}
\item{}
\item{(i)}The following are equivalent:
\begin{itemize}
\item $N \subset M$ is approximately extremal;
\item $\Trace'_{2i+1} \sim \Trace_{2i+1}$ for all $i \geq 0$;
\item $\Trace'_{2i+1} \sim \Trace_{2i+1}$ for some $i \geq 0$;
\item $\rho_k$ exists for all $k \geq 0$;
\item $\rho_k$ exists for some $k \geq 1$;
\item $\widetilde{\rho}_k$ exists for all $k \geq 0$;
\item $\widetilde{\rho}_k$ exists for some $k \geq 1$.
\end{itemize}
\item{(ii)} The following are equivalent:
\begin{itemize}
\item $N \subset M$ is extremal;
\item $\Trace'_{2i+1}=\Trace_{2i+1}$ for all $i \geq 0$;
\item $\Trace'_{2i+1}=\Trace_{2i+1}$ for some $i \geq 0$;
\item $\rho_k$ (or $\widetilde{\rho}_k$) exists for all $k \geq 0$ and
  is unitary
\item $\rho_k$ (or $\widetilde{\rho}_k$) exists for all $k \geq 0$ and
  $\rho=\widetilde{\rho}$;
\item $\rho_k$ (or $\widetilde{\rho}_k$) exists for some $k \geq 1$
  and is unitary
\item $\rho_k$ (or $\widetilde{\rho}_k$) exists for some $k \geq 1$
  and $\rho=\widetilde{\rho}$;
\end{itemize}
\end{description}
\end{thm}


==> inf/rotations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ROTATIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Rotations}
\label{sect: rotations}

\begin{definition}
\begin{description}
\item
\item{1.} Let $B$ be a $M_N$-basis.  If $\sum_{b \in B} R_{b^*} \br{
L_{b^*}}^* \hatt{x}$ converges for all $x \in N' \cap
\gothn_{\Trace_k}$ and extends to a bounded operator from $N' \cap
\Ltwo(M_k)$ to $\Ltwo(M_k)$ we define $\rho^B_k$ to be this extension.
\item{2.} Let $P_c=P_{N'\cap\Ltwo(M_k)}$.  If
\[
\br{x_1 \tensorN x_2 \tensorN \cdots \tensorN x_{k+1}}
\mapsto P_c\br{x_2 \tensorN x_3 \tensorN \cdots 
  \tensorN x_{k+1} \tensorN x_1}
\]
extends to a bounded operator on all $\Ltwo(M_k)$ we define
$\wtilde{\rho}_k$ to be this extension.
\end{description}
\end{definition}

\begin{thm}
\label{thm: rho, tilde(rho)}
If $\rho^B_k$ and $\rho^{\overline{B}}_k$ both exist then
$\rho^B_k=\rho^{\overline{B}}_k$.

If $\wtilde{\rho}_k$ exists then for any orthonormal basis $B$,
$\rho^B_k$ exists.  If $\rho^B_k$ exists for some $B$ then
$\wtilde{\rho}_k$ exists.  In this case both operators map $N' \cap
\Ltwo(M_k)$ onto $N' \cap \Ltwo(M_k)$.  Restricted to $N' \cap
\Ltwo(M_k)$ both are periodic (with period $k+1$) and
$\br{\rho^B_k}^*=\br{\wtilde{\rho}_k}^{-1}$.
\begin{proof}
\begin{description}
\item{1.} If $\rho^B_k$ exists then, as in the finite index case of
Section~\ref{sect: finite index IIone}, for $x \in N' \cap
\gothn_{\Trace_k}$ and $y=y_1 \tensorN \cdots \tensorN y_{k+1}$,
\begin{align}
\ip{\rho^B_k(x),y}
&=\sum_b \ip{x, L_{b^*} \br{ R_{b^*}}^* y} 
  \nonumber \\
&=\sum_b \ip{x, b^* \tensorN y_1 \tensorN \cdots \tensorN y_k E_N(y_{k+1}b)} 
  \nonumber \\
&=\sum_b \ip{xE_N(y_{k+1}b)^*,b^* \tensorN y_1 \tensorN \cdots \tensorN y_k} 
  \nonumber \\
&=\sum_b \ip{E_N(y_{k+1}b)^*x,b^* \tensorN y_1 \tensorN \cdots \tensorN y_k} 
  \nonumber \\
&=\sum_b \ip{x,E_N(y_{k+1}b)b^* \tensorN y_1 \tensorN \cdots \tensorN y_k} 
  \nonumber \\
&=\ip{x,y_{k+1} \tensorN y_1 \tensorN \cdots \tensorN y_k} .
  \label{eq: rho inner prod}
\end{align}
Hence $\rho^B_k(x)$ is independent of the basis used.  Note that
for $u\in \mathcal{U}(N)$
\begin{align*}
\sum_{b \in B} R_{(ub)^*} \br{ L_{(ub)^*}}^* \hatt{x}
&= \sum_{b \in B} R_{b^*u^*} \br{ L_{b^*u^*}}^* \hatt{x} \\
&= \sum_{b \in B} R_{b^*u^*} u \br{ L_{b^*}}^* \hatt{x} \\
&= \sum_{b \in B} u R_{b^*u^*} \br{ L_{b^*}}^* \hatt{x} \\
&= \sum_{b \in B} u \br{R_{b^*} \br{ L_{b^*}}^* \hatt{x} }\cdot u^* \\
&= u (\rho_k(\hatt{x}))\cdot u^* .
\end{align*}
So if $\rho^B_k$ exists then $\rho^{uB}_k$ exists and
$u\rho^B_k(\hatt{x})u^*=\rho^{uB}_k(\hatt{x})=\rho^B_k(\hatt{x})$.
Thus $\rho^B_k(\hatt{x}) \in N' \cap \Ltwo(M_k)$.  From~(\ref{eq: rho
inner prod}), $\br{\rho^B_k}^{k+1}=\id$.

In addition $P_c\br{y_2 \tensorlN \cdots \tensorlN y_{k+1} \tensorlN
y_1 }=\br{\br{\rho^B_k}^k P_c}^*\hatt{y}$, so that $\wtilde{\rho}_k$
exists.  On $N' \cap \Ltwo(M_k)$, $\wtilde{\rho}_k
=\br{\br{\rho^B_k}^{-1}}^*$.  Hence $\br{\wtilde{\rho}_k}^{k+1}=\id$ and
$\br{\rho^B_k}^*=\wtilde{\rho}_k^{-1}$.

\item{2.} If $\wtilde{\rho}_k$ exists then let $\sigma_k=\br{ P_c J_k
\wtilde{\rho}_k J_k P_c }^*$.  Take an orthonormal basis $\{ b \}
= \{ b_i \}$.  Then, reversing the argument in~(\ref{eq: rho inner
prod}), for $\xi \in N' \cap \Ltwo(M_k)$,
\begin{equation}
\label{eq: weak conv?}
\ip{\sigma_k(\xi),y}
=\sum_b \ip{R_{b^*} \br{L_{b^*}}^*\xi, y} ,
\end{equation}
Let $\eta=\sigma_k(\xi)$.  Note that $\eta_i \defeq R_{b_i^*}\br{
L_{b_i^*} }^* \xi$ are pairwise orthogonal.  For $y=y_1 \tensorlN
\cdots y_k \tensorlN b_i^*$ the sum in (\ref{eq: weak conv?}) only has
one term, so the equality extends by continuity to all
$R_{b_i^*}\zeta$ ($\zeta \in \Ltwo(M_{k-1})$) and in particular to
$\eta_i$.  Thus $\ip{\eta,\eta_i} =\ip{\eta_i, \eta_i}$ and so
\[
\sum_{i=1}^K ||\eta_i||^2
=\ip{\eta, \sum_{i=1}^K \eta_i} \\
\leq ||\eta|| \left|\left|\sum_{i=1}^K \eta_i\right|\right| \\
= ||\eta|| \br{ \sum_{i=1}^K ||\eta_i||^2 }^{1/2}
\]
which yields
\[
\br{\sum_{i=1}^K ||\eta_i||^2}^{1/2} \leq ||\eta|| .
\]
Hence $\sum_{i=1}^K ||\eta_i||^2$ is bounded, so $\sum_{i=1}^K \eta_i$
converges and by~(\ref{eq: weak conv?}) converges to $\eta$.  Hence
$\rho^B_k$ exists.
\end{description}
\end{proof}
\end{thm}

\begin{remark}
In Corollary~\ref{cor: rotn for one basis implies rotn for all} we
will see that if $\rho^B_k$ exists for some basis $B$ then it exists
for all bases and we will then drop the reference to $B$ and use the
notation $\rho_k$.
\end{remark}

